Qualitative and Quantitative Monitoring of Spatio-Temporal Properties with SSTL

In spatially located, large scale systems, time and space dynamics interact and drives the behaviour. Examples of such systems can be found in many smart city applications and Cyber-Physical Systems. In this paper we present the Signal Spatio-Temporal Logic (SSTL), a modal logic that can be used to specify spatio-temporal properties of linear time and discrete space models. The logic is equipped with a Boolean and a quantitative semantics for which efficient monitoring algorithms have been developed. As such, it is suitable for real-time verification of both white box and black box complex systems. These algorithms can also be combined with stochastic model checking routines. SSTL combines the until temporal modality with two spatial modalities, one expressing that something is true somewhere nearby and the other capturing the notion of being surrounded by a region that satisfies a given spatio-temporal property. The monitoring algorithms are implemented in an open source Java tool. We illustrate the use of SSTL analysing the formation of patterns in a Turing Reaction-Diffusion system and spatio-temporal aspects of a large bike-sharing system.

==> caseStudy.tex <==
% !TEX root =  main.tex

\section{SSTL Analysis of Stochastic Spatio-temporal Systems}
%%%\label{sec:caseStudy}
%%%
%%%
%%%In this section we show how SSTL can be used to identify the formation of \emph{patterns} in a reaction-diffusion system. 
%%%%not just that variables change over the time, but also that these are spatially organised. 
%%%Alan Turing conjectured in~\cite{turing_chemical_1952} that pattern formation is a consequence of the coupling of reaction and diffusion phenomena involving different chemical species, and that these can be described by a set of PDE reaction-diffusion equations, one for each species.The natural analogue, systems of agents interacting and moving in continuous space, is however prohibitively expensive to analyse computationally; an approach that is more amenable to analysis is to discretise space into a number of cells which are assumed to be spatially homogeneous, and to replace spatial diffusion with transitions between different cells.
%%%
%%%From the point of view of formal verification, the formation of patterns is an inherently spatio-temporal phenomenon, in that the relevant issue is how the spatial organisation of the system changes over time.
%%% 
%%%\subsection*{Pattern formation model}
%%%Our model, similar to ~\cite{bartocci2014, bartocci2015},  describes the production of skin pigments that generate spots in animal furs.
%%%The reaction-diffusion system is discretised, according to a Finite Difference scheme, as a system of ODEs whose variables are organised in a $K \times K$ rectangular grid.
%%%More precisely, we treat the grid as a weighted undirected graph, where each cell $(i,j) \in L = \{1,\ldots,K\} \times \{1,\ldots,K\}$ 
%%%%\mathbb{N}_{[1,K]} \times \mathbb{N}_{[1,K]}$ 
%%%is a location (node), edges connect each pairs of neighbouring nodes along four directions (so that each node has at most $4$ adjacent nodes), and the weight of each edge is always equal to the spatial length-scale $\delta$ of the system\footnote{For simplicity, here we fix $\delta=1$. Note that using a non-uniform mesh
%%%%, for instance obtained by a Finite Elements approach in PDE integration, 
%%%the weights of the edges of the resulting graph will not be uniform.}.
%%%We consider two species (chemical substances) $A$ and $B$ in a  $K \times K$ regular grid, obtaining the system:
%%%%$$
%%%%\begin{cases} 
%%%%\frac {\partial x_{A}}{\partial t} =  f(x_{A}, x_{B}) + D_{1} \triangle x_{A} \\
%%%%\frac {\partial x_{B}}{\partial t} =    g(x_{A}, x_{B}) + D_{2} \triangle x_{B}\\
%%%%\end{cases}
%%%%$$
%%%%where $x_{A}$ and $ x_{B}$ are the concentrations of the two species, $f$ and $g$ are the reaction functions, $D_{1}$ and $D_{2}$ are the diffusion constants and $\triangle$ is the laplaciano.
%%% \begin{equation}
%%%\begin{cases} 
%%%\frac {d x^{A}_{i,j}}{d t} =  R_{1} x^{A}_{i,j}  x^{B}_{i,j} - x^{A}_{i,j}  + R_{2} + D_{1} (\mu^{A}_{i,j} - x^{A}_{i,j}) &  i=1..,K, \mbox{ } j=1,..,K,\\  
%%%\frac {d x^{B}_{i,j}}{d t} =  R_{3} x^{A}_{i,j}  x^{B}_{i,j}  + R_{4}  + D_{2} (\mu^{B}_{i,j} -  x^{B}_{i,j}) & i=1..,K, \mbox{ }  j=1,..,K,\\
%%%\end{cases}
%%%\label{model}
%%% \end{equation}
%%%where: $x^{A}_{i,j}$ and $ x^{B}_{i,j}$ are the concentrations of the two species in the cell $(i,j)$;
%%%$R_{i}$, $i = 1,...,4$ are the parameters that define the reaction between the two species;
%%% $D_{1}$ and $D_{2}$ are the diffusion constants; $\mu^{A}_{i,j}$ and $\mu^{B}_{i,j}$ are the inputs for the $(i,j)$ cell, that is
%%% \begin{equation}
%%% \mu^{n}_{i,j}= \frac{1}{|\nu_{i,j} |} \sum_{\nu \in \nu_{i,j}} x^{n}_{\nu}   \qquad n \in \{ A, B\},
%%% \end{equation}
%%% where $\nu_{i,j}$ is the set of indices of cells adjacent to  $(i,j)$.
%%%The spatio-temporal trace of the system is the function $\vec x = (x^{A}, x^{B}) : [0, T] \times L\rightarrow \mathbb{R}^{K \times K} \times \mathbb{R}^{K \times K}$ where each $x^{A}$ and $x^{B}$ are the projection on the first and second variable, respectively.
%%% In Fig. \ref{sim} the concentration of species A is shown for a number of time points, generated by the numerical integration of System \ref{model}; at time $t=20$ and $t=50$, the shape of the pattern is apparent and remains stable. Clearly, some regions (in blue) have a low concentration of A surrounded by regions with a high concentration of A. We consider the regions with low concentration of species A as the `spots' in the pattern. The opposite happens for the value of B (high density regions surrounded by low density regions, not shown).
%%%
%%%\begin{figure}[tbp]
%%%\centering
%%%\includegraphics[width=1. \textwidth]{./figs/simulation}
%%%\caption{Value of $x^{A}$ for the system (\ref{model}) for $t=0, 5, 7, 12, 20,50$ time units with parameters $K=32, R_{1}=1, R_{2}=-12, R_{3}=-1, R_{4}= 16, D_{1} = 5.6$ and $D_{2}= 25.5.$  The initial condition has been set randomly. The colour map for the concentration is specified in the legend on the right.}
%%%\label{sim}
%%%\end{figure}

%\begin{figure}[ht]
%\centering
%\subfigure[t=0]{\label{simt0}{\includegraphics[width=0.15\textwidth]{./figs/simB0}}}\hfill
%%\hspace{-10mm}
%\subfigure[t=5]{\label{simt1}{\includegraphics[width=0.15\textwidth]{./figs/simB5}}}\hfill
%%\hspace{-10mm}
%\subfigure[t=7]{\label{simt2}{\includegraphics[width=0.15\textwidth]{./figs/simB7}}}\hfill
%%\hspace{-10mm}
%\subfigure[t=12]{\label{simt3}{\includegraphics[width=0.15\textwidth]{./figs/simB12}}}\hfill
%%\hspace{-10mm}
%\subfigure[t=20]{\label{simt4}{\includegraphics[width=0.15\textwidth]{./figs/simB20}}}\hfill
%%\hspace{-10mm}
%\subfigure[t=30]{\label{simt5}{\includegraphics[width=0.155\textwidth]{./figs/simB30leg}}}\hfill
%
%\caption{Simulation of the system \ref{model} for a number of time points with parameters $R_{1}=1, R_{2}=-12, R_{3}=-1, R_{4}= 16, D_{1} = 5.6$ and $D_{2}= 25.5.$  }
%\label{sim}
%\end{figure}
%\begin{equation}
%\mu_{1} : X_{B} >  K \mbox{, } \mu_{2} : X_{A}> H 
%\end{equation}
%
%\begin{equation}
% \phi_{Surround} : \mu_{1} S {[w_{1},w_{2}]} \mu_{2}
%\end{equation}

%%%\subsection{Spot and Pattern Formation properties}
%%%The following shows how we can use the surrounded operator to characterise the behaviour of this system.
%%% In order to classify spots, one should identify the sub-regions of the grid that present a high (or low) concentration of a certain species, surrounded by a low (high, respectively) concentration of the same species.  
%%% Formally, one can e.g., capture the spots of the A species using the spatial formula
%%% \begin{equation}
%%% \phi_{ \mathrm{spot}} := ( x^{A} \leq h   ) \surround{[d_{1},d_{2}]} ( x^{A} > h  ). 
%%%\end{equation}
%%%A trace $\vec{x}$ satisfies $\phi_{ \mathrm{spot}}$ at time $t$, in the location $(i,j)$, $(\vec{x},t, (i,j)) \models \phi_{ \mathrm{spot}}$, if and only if there is 
%%%%\marginpar{V: non comprendo la notazione $N_{1} \times N_{2}$ per denotare un sottoinsieme di un prodotto. Nessuno garantisce che un sottoinsieme arbitrario sia in quella forma. Questo paragrafo \`e un po' preliminare, ma ne parliamo per e-mail.} 
%%%a subset $L'\subset L$, that contains $(i,j)$, such that all elements in $L'$ have a distance less than $d_{2}$ from $(i,j)$, and $x^{A}$, at time $t$, is less or equal to $h$. Furthermore, in each element in the boundary of $L'$ we have that $x^A>h$ at time $t$, and its distance from $(i,j)$ is in the interval $[d_{1}, d_{2}]$. Note that the use of distance bounds in the surrounded operator allows one to constrain the size (diameter) of the spot.% to $[d_{1}, d_{2}]$.
%%%
%%%%\MNFA{The diameter or size should be a number and not an interval. Do you mean that the diameter is less than $d_2 -d_1$?}  
%%%%NO. The diameter of the spot is related to [d_1,d_2] but this does not completely characterise the size of the spot. 
%%%%
%%%%Indeed, a location $(i,j)$ inside a spot must reaches the boundary of the spot, in all the direction with a weight $w \in [w_{1}, w_{2}]$.
%%%Recall that we are considering a spatio-temporal system, so this spatial property alone is not enough to describe the formation of a pattern {\em over time}; to identify the insurgence time of the pattern and whether it remains stable over time we can combine the spatial property with  temporal operators in the following way:
%%%\begin{equation}
%%% \phi_{ \mathrm{spotFormation}} := \mathcal{F}_{[T_{ \mathrm{pattern}}, T_{ \mathrm{pattern}} + \delta]} \mathcal{G}_{[0,T_{ \mathrm{end}}]} ( \phi_{ \mathrm{spot}});
%%% \label{phi}
%%%\end{equation}
%%%$\phi_{ \mathrm{spotFormation}}$ states that eventually at a time between $T_{ \mathrm{pattern}}$ and  $T_{ \mathrm{pattern}} + \delta $ the property $\phi_{ \mathrm{spot}}$ becomes true and remains true for at least $T_{ \mathrm{end}}$ time units.
%%%%
%%%%In Fig. \ref{result} we can see the the boolean and the quantitative semantic in each location of the grid for the property $\phi$.
%%%Fig. \ref{result} shows the satisfaction of the property $\phi_{\mathrm{spotFormation}}$ in each cell $(i,j) \in L$, 
%%%for both the Boolean (Fig.~\ref{result}(b)) and the quantitative semantics (Fig.~\ref{result}(c)). The plots show the satisfaction at time $t = 0$ because by default we have that $(\vec x, \ell ) \models \varphi $, if and only if $ (\vec x,0, \ell) \models \varphi $.
%%%%
%%%%Recalling that  $(\vec x, \ell ) \models \varphi $, if and only if $ (\vec x,0, \ell) \models \varphi $,  for this reason the plots show the satisfaction at time $t = 0$.
%%%It is clear how well the procedure is able to identify which locations belong to the spots and which not. 
%%%If we make the distance constraint stricter, by reducing the width of the interval $[d_{1}, d_{2}]$, we are able to identify only the ``centre'' of the spot, as shown in Fig. \ref{result} (d). However, in this case we may fail to identify spots that have an irregular shape (i.e., that deviate too much from a circular shape). 
%%%
%%%Formula $\phi_{\mathrm{pattern}}$ describes the persistence of a spot in a specific location. To describe the global spatial pattern, that every location is part of a spot or has a nearby spot, the following SSTL formula can be used:
%%%\begin{equation}
%%%\phi_{\mathrm{pattern}} := \everywhere{[0,d_{max}]} \somewhere{[0,d_{spot}]}  \phi_{\mathrm{spot}}, 
%%%\label{phi:pattern}
%%%\end{equation}
%%% where $\diamonddiamond$ and $\boxbox$ are the everywhere and somewhere operators, $d_{max}$ is chosen to cover all space, and $d_{spot}$ measures the maximal distance between spots. Checking this formula in a random location of our space is enough to verify the presence of the pattern; this is so because the first part of the formula, $\everywhere{[0,d_{max}]}$, covers all the locations of the grid. This is an example of how one can describe a global property also with a semantics that verifies properties in single locations. We verify property (\ref{phi:pattern}) with $d_{max}=45$ and $d_{spot}=15$ (the other parameters are as indicated in Fig.~\ref{result}), for a solution of the system (\ref{model}) obtaining true for the Boolean semantics and  $0.3$ for the quantitative one. The low value of the quantitative semantics is due to the choice of the threshold $h$.
%%%
%%%\begin{figure}[tbp]
%%%\centering
%%%\includegraphics[width=1. \textwidth]{./figs/check}
%%%\caption{Satisfaction of formula (\ref{phi}) with $h=0.5, T_{\mathrm{pattern}}= 19, \delta = 1, T_{\mathrm{end}} =30,  w_{1}=1, w_{2}=6$ for (b), (c) and $w_{2}=4$ for (d). (a) Concentration of $A$ at time t = 50; (b) (d) Boolean semantics of the property $\phi_{\mathrm{pattern}}$; the cells (locations) that satisfy the formula are in red, the others are in blue;
%%%(c) Quantitative semantics of the property $\phi_{\mathrm{pattern}}$; The value of the robustness is given by a colour map as specified in the legend on the right of the figure.}
%%%\label{result}
%%%\end{figure}
%%%%Changing the diffusion constants $D_{1}$ and $D_{2}$ affects the shape and size of spots or disrupt their formation, as can be seen in Fig. \ref{resultNoPattern} (a). In this case, we expect formula (\ref{phi}) to be false in all locations. This is indeed the case, excluding boundary effects on the border of the grid (where only a fraction of spots remains, see e.g., Fig. \ref{resultNoPattern} (a) right). 
%%%%We check the same formula, with the stronger distance constraint, for the same model (\ref {model}) with different value of parameters $D_{1}$ and $D_{2}$, where the result simulations do not present the same pattern as the previous system, a snapshot of these simulations can be seen in Fig. . The boolean semantics is equal to zero in almost all the locations, except some locations in the border satisfies the property (because the rest of their spots is ``out'' of the system), the quantitative semantics are in ranges $[],[],[]$ in the three different cases.  
%%%%
%%%%Changing the diffusion constants $D_{1}$ and $D_{2}$ affects the shape and size of the spots or disrupts them  (Fig. \ref{resultNoPattern} (a)). We evaluate formula (\ref{phi:pattern}) for model  (\ref{model}) with parameters $D=[1.5, 23.6]$ and $D=[8.5, 40.7]$,  as in Fig. \ref{result} (a), and it results false with a quantitative value equal to -0.05 for both. Formula
%%%% (\ref{phi}),  instead,  is still true in some locations.  This is due to the irregularity of the spots (where, as Fig. \ref{resultNoPattern} (a) left, some spots can have a shape similar to the model in Fig. \ref{result} (a)), or due to particular boundary effects on the border of the grid (where fractions of spots still remain, as in Fig. \ref{resultNoPattern} (a) right). 
%%%
%%%Changing the diffusion constants $D_{1}$ and $D_{2}$ affects the shape and size of the spots or disrupts them, as we can see in Figure~\ref{fig:NoPattern}. We evaluate the pattern formula (\ref{phi:pattern}) with parameters as in Fig.~\ref{result}, for the patterns in Figure~\ref{fig:NoPattern},
%%%where $D=[1.5, 23.6]$ and $D=[8.5, 40.7]$ and the other parameters equal to the previous model, and it results false with a quantitative value equal to -0.05 for both. Formula
%%% (\ref{phi}),  though,  is still true in some locations.  This is due to the irregularity of the spots (where, as in Fig.~\ref{fig:nopattern1}, some spots can have a shape similar to the model in Fig.~\ref{result} (a)), or due to particular boundary effects on the border of the grid (where fractions of spots still remain, as in Fig. \ref{fig:nopattern1}). 
%%%  
%%%\begin{figure}[!t]
%%%\begin{center}
%%%%\subfigure[Snapshot]{
%%%%\label{fig:1}
%%%%%\includegraphics[width=.485\textwidth]{figs/trajoptI1FFL.pdf} }
%%%%\includegraphics[width=.31\textwidth]{snapshot} 
%%%%}
%%%\subfigure[]{
%%%\label{fig:nopattern1}
%%%%\includegraphics[width=.485\textwidth]{figs/trajoptI1FFL.pdf} }
%%%\includegraphics[width=.4\textwidth]{./figs/noPattern1} 
%%%}
%%%\subfigure[]{
%%%\label{fig:nopattern2}
%%%%\includegraphics[width=.48\textwidth]{figs/distoptI1FFL.pdf} }
%%%\includegraphics[width=.4\textwidth]{./figs/noPattern2} 
%%%}
%%%\end{center}
%%%\caption[Snapshots of the model with %parameters 
%%%``bad'' diffusion rate D]{Snapshots at time $t=50$ of $x^A$ for the model (\ref{model}) with parameters with parameters $K=32, R_{1}=1, R_{2}=-12, R_{3}=-1, R_{4}= 16$, and $D=[1.5, 23.6]$ in (a) and $D=[8.5, 40.7]$ in (b).}
%%%%\vspace{-0.4cm}
%%%\label{fig:NoPattern}
%%%\end{figure}
 
%%%\subsection{Perturbation property}A strength of spatio-temporal logics is the possibility to nest the temporal and spatial operators. We illustrate this in the following scenario. We set as  initial conditions for the system (\ref{model}) its stable state, i.e. the concentrations of $A$ and $B$ at time $50$ (see Fig. \ref{result}(a)). We introduce a small perturbation, by changing a single value in a specific location in the centre of a spot. The idea is to study the effect of this perturbation, i.e., checking whether it will disrupt the system or not. Specifically, we perturb the cell $(6,6)$ in Fig.~\ref{result}(a), by setting  $x_{6,6}^{A}(0)=10$ while its original value was 0. Dynamically, the perturbation is quickly absorbed and the system returns to the previous steady state. Formally, we consider the following property:
%%%%We formally investigate this scenario by checking the following property:
%%%{
%%%\begin{equation}
%%% \phi_{\mathrm{pert}} :=(x^{A}\geq h_{\mathrm{pert}}) \wedge(\phi_{\mathrm{absorb}} \surround{[d_{m},d_{M}]} \phi_{\mathrm{no\_effect}}); 
%%%%    (x^{A}\geq h_{p}) \
%%%%          \phi_{1} := \mathcal{F}_{[0, T_{p}]} \mathcal{G}_{[0, T_{d}]} (  x_{A} < h'); \
%%%%           \phi_{2} := \mathcal{G}_{[0, T]} (  x^{A} < h' );
%%% \label{phi_pert}
%%%\end{equation}
%%%}
%%%$ (\vec x, (i,j)) \models \phi_{\mathrm{pert}}$, i.e., a trace $\vec{x}$ satisfies $\phi_{\mathrm{pert}}$ in the location $(i,j)$, if and only if $x_{i,j}^{A}(0) > h_{\mathrm{pert}} $ (the location is perturbed) and if there is a subset $L' \subseteq L$ that contains $(i , j)$ such that all its elements have a distance less than $d_{M}$ from $(i,j)$ and satisfy $\phi_{\mathrm{absorb}}=  \mathcal{F}_{[0, T_{p}]} \mathcal{G}_{[0, T_{d}]} (  x^{A} < h')$; $\phi_{\mathrm{absorb}}$ states that the perturbation of $x^A$ is absorbed within $T_p$ units of time, stabilising back to a value $ x^{A} < h'$ for an additional period of $T_{d}$ time units.
%%%Furthermore, within distance $[d_{m}, d_{M}]$ from the original perturbation, where $d_M$ is chosen such that we are within the spot of the non-perturbed system, $\phi_{\mathrm{no\_effect}} := \mathcal{G}_{[0, T]} (  x^{A} < h' )$ is satisfied; i.e., no relevant effect is observed, the value of $x^A$ stably remains below $h'$.  The meaning of $\phi_{\mathrm{pert}}$ is that the induced perturbation remains confined inside the original spot.
%%%In Fig. \ref{perturb}, we report the evaluation of the quantitative semantics for $\phi_{\mathrm{pert}}$, zooming in on the $15\times 15$ lower left corner of  the original grid. As shown in the figure, the perturbed location $(6,6)$ satisfies the property.
%%%
%%%\VNFA{Ho modificato la figura 8 (che era un unico pdf per 2 figure) per poter usare il subfigure. Per farlo ho importato il pdf (!!) in inkscape e le ho separate. Nota bene: nella figura si vede un effetto ``collage'' nel pdf in alcuni viewer, ma questo era presente già prima; l'immagine originale sembra essere composta di vari pezzettini tagliati e incollati, probabilmente il programma che l'ha prodotta introduce questo tipo di cose. Ancora: i pixel sono 14 anche se la numerazione arriva a 15. Ho anche ridotto la dimensione delle etichette numeriche e duplicato le scale per consistenza col resto. Volendo si può anche rifare la figura con lo strumento usato originariamente; ma a me sembra che così possa andare. Comunque trovate gli svg nel repository nella stessa directory della figura.}
%%%
%%%% 
%%%%  \begin{figure}[tbp]
%%%% \centering
%%%% \includegraphics[width=.8 \textwidth]{./figs/perturb}
%%%%  \vspace{-7mm}
%%%%  
%%%%  
%%%\begin{figure}[!t]
%%%\begin{center}
%%%%\subfigure[Snapshot]{
%%%%\label{fig:1}
%%%%%\includegraphics[width=.485\textwidth]{figs/trajoptI1FFL.pdf} }
%%%%\includegraphics[width=.31\textwidth]{snapshot} 
%%%%}
%%%\subfigure[]{
%%%\label{perturbA}
%%%%\includegraphics[width=.485\textwidth]{figs/trajoptI1FFL.pdf} }
%%%\includegraphics[height=9em]{./figs/perturbA.pdf} 
%%%}
%%%\hskip 20pt
%%%\subfigure[]{
%%%\label{perturbB}
%%%%\includegraphics[width=.48\textwidth]{figs/distoptI1FFL.pdf} }
%%%\includegraphics[height=9em]{./figs/perturbB.pdf} 
%%%}
%%%\end{center} 
%%%\caption {Boolean (a) and quantitative (b) semantics for formula~\ref{phi_pert}  with parameters 
%%%$h_{\mathrm{pert}} = 10$, $w_m =1$, $w_M=2$, $T_p=1$, $T_d = 10$, $h'=3$, and $T=20$.} 
%%%%
%%%%Concentration of A at time t=50 for the system (\ref{model}) with different values of  $\vec D = [D_{1} , D_{2}]$. The other parameters remain equal of the previous simulations.  (a)  $\vec D=[0.2, 20] $; (b)  $\vec D=[1.4, 5.3] $; (c)  $\vec D=[2.5, 10.7] $; The value of the concentration is given by the colour as specified in the legend on the right of the figure.
%%%\label{perturb}
%%%\vspace{-3ex}
%%%\end{figure}
%%%
%%%
%%%% \begin{figure}[tbp]
%%%%\centering
%%%%\includegraphics[width=1. \textwidth]{./figs/noPattern_perturb}
%%%%\caption{(a) Snapshots at time $t=50$ of $x^A$ for the model (\ref{model}) with %parameters 
%%%%$D=[1.5, 23.6]$ (on the left) and $D=[8.5, 40.7]$ (on the right).
%%%%(b) Boolean and quantitative semantics for the formula $\phi_{\mathrm{pert}}$ with %parameters 
%%%%$h_{\mathrm{pert}} = 10$, $w_m =1$, $w_M=2$, $T_p=1$, $T_d = 10$, $h'=3$, and $T=20$.} 
%%%%%
%%%%%Concentration of A at time t=50 for the system (\ref{model}) with different values of  $\vec D = [D_{1} , D_{2}]$. The other parameters remain equal of the previous simulations.  (a)  $\vec D=[0.2, 20] $; (b)  $\vec D=[1.4, 5.3] $; (c)  $\vec D=[2.5, 10.7] $; The value of the concentration is given by the colour as specified in the legend on the right of the figure.
%%%%\label{resultNoPattern}
%%%%\end{figure}


%\subsection{Stochastic system}
\VNFA{Modificato per rispondere ad un commento dei revisori, fatemi sapere se secondo voi occorre aggiungere altro.}
SSTL can also be applied to describe properties of stochastic spatio-temporal systems. We propose a \emph{statistical model checking} approach. Statistical model checking is a verification technique for stochastic systems that employs a qualitative (that is, non-probabilistic) model checker, which is capable of verifying the satisfaction of a given formula $\Phi$ \emph{on a specific system run}, to return an answer to the question ``what is the probability that an arbitrary run of the system satisfies $\phi$ with a certain degree of confidence''? Informally speaking, in order to do so, several probabilistic simulations of the system are computed, and the formula $\Phi$ is tested using the qualitative model checker on each obtained run. The positive and negative outcomes of the model checking algorithm are then counted, and statistical methods are used to compute the degree of confidence and probability obtained.

Similarly to the methodology developed in \cite{CLMPV16}, the monitoring algorithms for SSTL can be plugged in seamlessly (in the informal explanation above, playing the role of the qualitative model checker) into existing statistical model checking routines.
In the following we present an example of this possibility.
We consider the effects of external perturbations of the system, adding a white Gaussian noise to the set of equations (\ref{model}).  In particular, we add a random fluctuation $\eta( \vec z, t)$, with zero-mean and covariance matrix
$<\eta(\vec z,t),\eta(\vec{z}',t)> = \epsilon^2 \delta z^2 \delta t$, where $\epsilon$ is the noise intensity and $\vec z = (i,j) \in [0, 32]^2$ corresponds to the position.
%, and then $\eta_{t+1} = \eta_t + \Delta \eta = \eta_t + \sqrt{\delta t} * A * randn$
The methodology follows \cite{lesmes_noise-controlled_2003,leppanen_effect_2003}.  In the discretisation, we set $\Delta z = 1$ and $\Delta t =0.01$.

We study how the noise affects the dynamics for fixed deterministic 
parameters, analysing in detail the capability of the system to maintain a specific pattern respect to the external perturbation. 
To this aim, we fix the parameters of the system:  $K=32, R_{1}=1, R_{2}=-12, R_{3}=-1, R_{4}= 16, D_{1} = 5.6$ and $D_{2}= 25.5$ and we 
evaluate formula \ref{phi:pattern} (the pattern formula) with parameters
 $h=0.5, T_{\mathrm{pattern}}= 19, \delta = 1, T_{\mathrm{end}} =30,  w_{1}=1, w_{2}=6$ for different values of the noise intensity $\epsilon$.
 
In Fig.~\ref{fig:prob},
we show how the satisfaction probability decreases as a function of the noise intensity $\epsilon$; $\epsilon$ was varied between $0$ and $0.9$ in steps of 0.1 units.  We estimate the probability statistically from $10,000$ runs for each parameter value.
%, (all results reported at 95\% confidence).


In Fig.~\ref{fig:probvsRob}, 
 we plot the satisfaction probability versus the average 
robustness degree, estimating them statistically from $10,000$ runs for each parameter value. The satisfaction probability varies from  1 to 0 while the average robustness score varies from $-80.01  \pm 10.7$ to $0.008  \pm 0$.
As we can see, these two quantities seem to be correlated.
By varying the threshold, the Pearson's correlation coefficient %CITE  
between satisfaction probability and robustness degree is $0.784$.
%, with an evident linear trend. 


  \begin{figure}[!t]
\begin{center}
%\subfigure[Snapshot]{
%\label{fig:1}
%%\includegraphics[width=.485\textwidth]{figs/trajoptI1FFL.pdf} }
%\includegraphics[width=.31\textwidth]{snapshot} 
%}
\subfigure[]{
\label{fig:prob}
%\includegraphics[width=.485\textwidth]{figs/trajoptI1FFL.pdf} }
\includegraphics[width=.465 \textwidth]{./figs/probPlot}
}
\subfigure[]{
\label{fig:probvsRob}
%\includegraphics[width=.48\textwidth]{figs/distoptI1FFL.pdf} }
\includegraphics[width=.44 \textwidth]{./figs/probvdRob}
}
\subfigure[]{
\label{fig:averageRob}
%\includegraphics[width=.48\textwidth]{figs/distoptI1FFL.pdf} }
\includegraphics[width=.45 \textwidth]{./figs/averageRob}
}
\end{center}
\caption{ (a) Satisfaction probability vs. noise intensity; (b) Satisfaction probability vs. average robustness degree; (c) Emprical distribution of the robustness degree for $\epsilon=0.1$.}
%\vspace{-0.4cm}
\label{fig:}
\end{figure}
 
  In Fig.~\ref{fig:averageRob}, we show the empirical distribution from 10,000 runs of the robustness degree for $\epsilon=0.1$, with vertical lines denoting the average (red lines) and conditional averages on the formula being false/ true (green lines). 
 

%%%\subsection{Implementation}
%%%Model (\ref{model}) has been coded in Matlab/Octave, and the monitoring has been performed by our Java implementation. 
%%%%
%%%As time performance, 
%%%%To give an indication of time performance, 
%%%the verification of property $\phi_{\mathrm{spot}}$ took $1.04s$ (boolean) and $69.39s$ (quantitative) for all locations and 100 time points, while property $\phi_{\mathrm{pattern}}$ took $1.81s$ and $70.06s$, and property $\phi_{\mathrm{pert}}$ took $28,19s$ and $55,31s$, respectively. The computation of the distance matrix can be done just once because it remains always the same for a given system, this takes about $23s$.
%%% All the experiments were run on an 
%%% %Macbook Pro, OS X 10.9.5, 
%%% Intel Core i5  2.6 GHz CPU, with 8GB 1600 MHz RAM.

%\begin{figure}[ht]
%\centering
%\subfigure[]{\label{pertSim}{\includegraphics[width=.5 \textwidth]{./figs/simPert2}}}\hfill
%%\hspace{-10mm}
%\subfigure[]{\label{pertCheck}{\includegraphics[width=.5\textwidth]{./figs/checkPert2}}}
%\caption{  }
%\label{}
%\end{figure}


% \marginpar{L: not sure this is formula is helpful. We need to think of additional, cooler, properties for this example} 
%The fact that atomic propositions are multi-dimensional permits one to provide multi-criteria specifications; e.g., the following formula identifies areas where the concentration of B is high and the concentration of A is low, surrounded by areas with low concentration of B and high concentration of A.
%
%
%
%\begin{equation}
% \phi_{Surround_{2}} : ( X_{B} \geq  K \wedge X_{A} <  H ) S {[w_{1},w_{2}]} ( X_{B} < K \wedge X_{A} \geq H )
%\end{equation}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

